Conditional Dependence via Shannon Capacity: Axioms, Estimators and Applications

We conduct an axiomatic study of the problem of estimating the strength of a known causal relationship between a pair of variables. We propose that an estimate of causal strength should be based on the conditional distribution of the effect given the cause (and not on the driving distribution of the cause), and study dependence measures on conditional distributions. Shannon capacity, appropriately regularized, emerges as a natural measure under these axioms. We examine the problem of calculating Shannon capacity from the observed samples and propose a novel fixed-$k$ nearest neighbor estimator, and demonstrate its consistency. Finally, we demonstrate an application to single-cell flow-cytometry, where the proposed estimators significantly reduce sample complexity.

==> intro.tex <==
\section{Introduction}

Knowledge bases (KB) store complex structured information by organizing {\em entities} in a directed graph: each node represents one entity, and two entities are connected by a {\em relation}, e.g., ({\sffamily \small Harry\_Potter}, instance of, {\sffamily \small Novel\_Series}). Popular KBs include Freebase \cite{bollacker2008freebase}, WordNet \cite{miller1995wordnet}, BabelNet \cite{navigli2010babelnet}, and Wikidata \cite{vrandevcic2014wikidata}. By their very nature, these KBs are incomplete and, at times, coarse/ambiguous.  Given the central utility of KBs in NLP and IR tasks,  completion and refining of KBs are first order issues.  This issue is addressed via harvesting relational facts via crowdsourcing, collating information across different existing KBs, and {\em unsupervised} extraction of relational facts directly from {\em unstructured} resources.  The last approach is very promising (due to its lack of expert human intervention) but also very challenging algorithmically. This paper addresses the major challenges of this approach,  where we extract facts from Wikipedia. 

The title of each page represents the concepts  in Wikipedia and has strong intersection with  the entities in KBs;  in the rest of paper we will use the word ``entity" to refer to both a concept in Wikipedia and an entity in KBs. In this  paper we propose a novel solution to extend KBs from the unstructured articles associated with each entity by extracting the {\em low dimensional representations} for entities from annotations and reasoning the relations between those in an unsupervised manner -- our effort is a conceptual departure from YAGO, which relies on harnessing the {\em structured }information in Wikipedia (e.g.\ categories, infoboxes, and redirects)  \cite{suchanek2007yago,hoffart2013yago2,mahdisoltani2014yago3} with the same end-goal and with inherently limited success. 

The ambiguous nature of words is the very essence of natural language \cite{lesk1986automatic}. A solution to resolve this ambiguity   is by representing words by multiple vectors, each corresponding to its unique sense \cite{huang2012improving,rothe2015autoextend}. In this study, we observe that just like words, relations between entities defined in KBs, can be ambiguous as well. Our approach to unsupervised entity representations  suggests an innovative unsupervised solution to disambiguate relations via  clustering triples. This leads to an immediate unsupervised and automatic refinement of the KB -- an  unexpected outcome of entity embeddings -- and one of the important findings of this paper. 

%\paragraph{Formulations.}
A large number of the entity mentions in Wikipedia are explicitly annotated to their corresponding documents through the use of links. We find the annotations to be ``natural language'' of semantics, and we learn a set of entity representations by parsing the annotations. This is a significant departure from prior work on entity representations, which have focused on reasoning the relatedness of entities from either their co-occurrence statistics (such as word-document co-occurrence) or their hyperlink structure from the extensive network of cross-references in Wikipedia  \cite{gabrilovich2007computing,dumais2004latent,witten2008effective,lesk1986automatic}. We improve upon these works by observing a tantalizing connection between annotation process and natural language: both are generated by humans for human consumption. In particular, we observe that the distributional hypothesis \cite{firth1957synopsis} for natural language holds for annotations as well: an entity is characterized by the company it keeps. Motivated by the ability of word2vec to capture analogies by the difference vectors of two word representations \cite{mikolov2013efficient}, we treat relational facts in KB as generalized analogies and wonder if the corresponding  entity representations can capture relatedness and relational facts as well.  The fact that they do is a central {\bf conceptual finding} of this paper. 

%\paragraph{Mathematical results.}
To obtain the entity representations, we study annotations via  a log-linear discriminative model (MODELNAME). Motivated by empirical observations of the natural language of annotations, we hypothesize that the parameters of the log-linear discriminative model are **** -- and show that such models are {\em self-normalizing} for almost every generative process. Here normalization refers to the computationally cumbersome step to ensure the model outputs valid probability distributions (and is they computational burden in the otherwise success-story of log-linear models for language modeling \cite{rosenfeld1996maximum,mnih2007three,mikolov2013efficient}, machine translation \cite{devlin2014fast}, and speech recognition \cite{graves2013hybrid}).  Self-normalization refers to the fact that the log-linear model outputs valid probability distributions despite no effort to explicitly normalize the outputs (and explored in recent works  \cite{andreas2014and}).   Our result explains self-normalization in the context of a large class of  log-linear models and represents the main {\bf mathematical contribution} of this paper; this result is also of independent mathematical interest.  Given that MODELNAME is self-normalizing, we propose a maximum likelihood formulation (christened {\em wiki2vec}) to estimate the parameters -- the entity embeddings -- using standard adaptive gradient descent. 
%in the tradition of method of moments 


The resulting entity representations strongly capture semantic relatedness and we demonstrate this  by evaluating its performance on two well-defined tasks. First, we study the semantic relatedness task, where one is asked to measure the similarity between entities, wiki2vec outperforms state-of-the-art on the KORE-20 dataset. An analogy task involves predicting $e_d$ given $e_a$, $e_b$, and $e_c$ such that $e_a$ is to $e_b$ is $e_c$ is to $e$, i.e., $e_a:e_b :: e_c:e_d$. This assumes $e_a$ and $e_b$ are to be linked by a relation and the same relation used to link $e_c$ and $e_d$. Second, we study wiki2vec on the  semantic analogy dataset in \cite{mikolov2013efficient} and show improved coverage of the questions {\em and} better prediction results. Finally,  we demonstrate strong KB completion,  via performing link prediction tasks on FB15k \cite{bordes2013translating}, and on a custom-built KB dataset derived from Wikidata. We conclude from this performance that it is possible to {\em encode and refine} link information contained in a KB in an {\em unsupervised} way, despite that the KB being  a highly supervised and structured dataset created entirely via (expert) human annotation; this is the main {\bf empirical contribution} of this paper. 

%In summary, the main contributions of this paper are the following:
%\begin{itemize}[leftmargin=*, nolistsep]
%\item We propose a log-linear discriminative model for annotations that is self-normalizing and an efficient training algorithm;
%\item We show that the latent representations are semantically meaningful. As a consequence, one can measure the relatedness accordingly and can infer structured resources like a KB from an unstructured corpus such as the Wikipedia;
%\item We observe the ambiguous behavior of relations in KBs, and propose an efficient method to refine them.
%\end{itemize}


